An Efficient Second-Order Accurate and Continuous Interpolation for Block-Adaptive Grids

In this paper we present a second-order and continuous interpolation algorithm for cell-centered adaptive-mesh-refinement (AMR) grids. Continuity requirement poses a non-trivial problem at resolution changes. We develop a classification of the resolution changes, which allows us to employ efficient and simple linear interpolation in the majority of the computational domain. The benefit of such approach is higher efficiency. The algorithm is well suited for massively parallel computations. Our interpolation algorithm allows extracting jump-free interpolated data distribution along lines and surfaces within the computational domain. This capability is important for various applications, including kinetic particles tracking in three dimensional vector fields, visualization (i.e. surface extraction) and extracting variables along one-dimensional curves such as field lines, streamlines and satellite trajectories, etc. Particular examples of the latter are models for acceleration of solar energetic particles (SEPs) along magnetic field-lines. As such models are sensitive to sharp gradients and discontinuities the capability to interpolate the data from the AMR grid to be passed to the SEP model without producing false gradients numerically becomes crucial. The code implementation of our algorithm is publicly available as a Fortran 90 library.

==> Previous_work.tex <==
Again, the numerical results obtained by control volume method in conjunction 
with AMR are sampled on the cell-centered grid.
To visualize data, one way is to resample them 
to corner-centered grid as done by many 
visualization tools, such as Tecplot.
However, this approach involves more distant grid cells
and, as a result, smoothens the data.
Alternative way is to visualize the uniform parts of the AMR grid directly
and to create a smooth transition between 
parts of the grid at different resolution levels.
To do so in \cite{Weber2001DataVis,Weber2001VMV,Moran2011IEEE},
the authors developed a stitching algorithm, as described in details in \cite{Weber2001DataVis}.

Their method achieves continuity and the second order of accuracy.
However, although good for visualization process, 
the algorithm isn't the most efficient for massive parallel computations,
since it is excessively branched.
This degrades its performance, hence, 
it would degrade the performance of the overall simulation,
should it be repeatedly applied at each time step.
As described further, this method is double-branched in two dimensions (2D)
and triple-branched in 3D, while our algorithm stays uniform.
Therefore the latter is preferable for 
repeated interpolation during the simulation.


